Reachability Analysis for Linear Systems with Uncertain Parameters using Polynomial Zonotopes

In real world applications, uncertain parameters are the rule rather than the exception. We present a reachability algorithm for linear systems with uncertain parameters and inputs using set propagation of polynomial zonotopes. In contrast to previous methods, our approach is able to tightly capture the non-convexity of the reachable set. Building up on our main result, we show how our reachability algorithm can be extended to handle linear time-varying systems as well as linear systems with time-varying parameters. Moreover, our approach opens up new possibilities for reachability analysis of linear time-invariant systems, nonlinear systems, and hybrid systems. We compare our approach to other state of the art methods, with superior tightness on two benchmarks including a 9-dimensional vehicle platooning system. Moreover, as part of the journal extension, we investigate through a polynomial zonotope with special structure named multi-affine zonotopes and its optimization problem. We provide the corresponding optimization algorithm and experiment over the examples obatined from two benchmark systems, showing the efficiency and scalability comparing to the state of the art method for handling such type of set representation.

==> temp.tex <==
Suppose we have a Multi-Affine polynomial \( p \) and its associated dependency graph \( G = (V, E) \). If \( G \) can be divided into different connected components \( G_1 = (V_1, E_1), G_2 = (V_2, E_2), \ldots, G_m = (V_m, E_m) \), then the optimization problem can be expressed as a sum of optimizations over each connected component:
\[
\min_{\alpha_i \in [-1,1],i \in V} p = \min_{\alpha_i \in [-1,1],i \in V_1} p_1 + \min_{\alpha_i \in [-1,1],i \in V_2} p_2 + \cdots + \min_{\alpha_i \in [-1,1],i \in V_m} p_m
\]
The running time for minimizing each subproblem is generally less than minimizing the original problem. Let's illustrate this with the following example:

\begin{example}
Consider a Multi-Affine polynomial \( p \) and its associated dependency graph \( G = (V, E) \) defined as follows:
\begin{align*}
    p &= a_1 \alpha_1 \alpha_2 \alpha_3 + a_2 \alpha_3 \alpha_4 + a_3 \alpha_5 \alpha_6 + a_4 \alpha_7, \\
    V &= \{\alpha_1, \alpha_2, \alpha_3, \alpha_4, \alpha_5, \alpha_6, \alpha_7\}, \\
    E &= \{\{\alpha_1, \alpha_2\}, \{\alpha_1, \alpha_3\}, \{\alpha_2, \alpha_3\}, \{\alpha_3, \alpha_4\}, \{\alpha_5, \alpha_6\}\}. % Edges are pairs that are part of a hyperedge in the Multi-Affine polynomial
\end{align*}

The dependency graph \( G \) can be divided into the following connected components:
\begin{itemize}
    \item \( G_1 = (V_1, E_1) \) with \( V_1 = \{\alpha_1, \alpha_2, \alpha_3, \alpha_4\} \) and \( E_1 = \{\{\alpha_1, \alpha_2\}, \{\alpha_1, \alpha_3\}, \{\alpha_2, \alpha_3\}, \{\alpha_3, \alpha_4\}\} \),
    \item \( G_2 = (V_2, E_2) \) with \( V_2 = \{\alpha_5, \alpha_6\} \) and \( E_2 = \{\{\alpha_5, \alpha_6\}\} \),
    \item \( G_3 = (V_3, E_3) \) consisting of the isolated vertex \( V_3 = \{\alpha_7\} \) with no edges.
\end{itemize}

The polynomial \( p \) can be decomposed into subpolynomials \( p_1 \), \( p_2 \), and \( p_3 \) corresponding to these components:
\begin{align*}
    p_1 &= a_1 \alpha_1 \alpha_2 \alpha_3 + a_2 \alpha_3 \alpha_4, \\
    p_2 &= a_3 \alpha_5 \alpha_6, \\
    p_3 &= a_4 \alpha_7.
\end{align*}

Thus, the original optimization problem can be decomposed into:
\[
    \min_{\alpha_i \in [-1,1], i \in V} p = \min_{\alpha_1, \alpha_2, \alpha_3, \alpha_4 \in [-1,1]} p_1 + \min_{\alpha_5, \alpha_6 \in [-1,1]} p_2 + \min_{\alpha_7 \in [-1,1]} p_3.
\]
Using the divide-and-conquer algorithm, we would enumerate \( 2^7 = 128 \) possibilities; however, by observing the decomposition into connected components, we only need to enumerate \( 2^4 + 2^2 + 2 = 22 \) possibilities, which is a significant reduction.
\end{example}
However, if the associated dependency graph is already a connected component, we propose to remove the vertex so that the dependency graph  can be partitioned into multiple connected. Let us illustrate it by considering the following example:

\begin{example}
Consider the Multi-Affine polynomial optimization problem defined by the polynomial:
\[
p(\alpha_1, \alpha_2, \alpha_3, \alpha_4, \alpha_5, \alpha_6, \alpha_7) = a_1 \alpha_1 \alpha_2 \alpha_3 + a_2 \alpha_3 \alpha_4 \alpha_5 + a_3 \alpha_2 \alpha_6 + a_4 \alpha_5 \alpha_7,
\]
where \( a_1, a_2, a_3, \) and \( a_4 \) are real coefficients. The associated dependency graph \( G = (V, E) \) for this polynomial is given by:
\begin{itemize}
    \item \( V = \{\alpha_1, \alpha_2, \alpha_3, \alpha_4, \alpha_5, \alpha_6, \alpha_7\} \)
    \item \( E = \{ \{\alpha_1, \alpha_2\}, \{\alpha_1, \alpha_3\}, \{\alpha_2, \alpha_3\}, \{\alpha_3, \alpha_4\}, \{\alpha_3, \alpha_5\}, \{\alpha_2, \alpha_6\}, \{\alpha_5, \alpha_7\} \} \)
\end{itemize}

In this dependency graph, vertex \( \alpha_3 \) is a key node connecting multiple edges. The removal of \( \alpha_3 \) leads to a partition of the graph into separate connected components. The remaining graph, after removing \( \alpha_3 \), is characterized by:

\begin{itemize}
    \item \( V' = \{\alpha_1, \alpha_2, \alpha_4, \alpha_5, \alpha_6, \alpha_7\} \)
    \item \( E' = \{ \{\alpha_1, \alpha_2\}, \{\alpha_4, \alpha_5\}, \{\alpha_2, \alpha_6\}, \{\alpha_5, \alpha_7\} \} \)
\end{itemize}

This results in two distinct connected components:
\[
V_1 = \{\alpha_1, \alpha_2, \alpha_6\}, \quad V_2 = \{\alpha_4, \alpha_5, \alpha_7\}.
\]
More specifically, if $\alpha_3 = 1$
\begin{align*}
   \min_{\alpha_i \in \{-1,1\},\alpha_3 = 1} p = \min_{\alpha_1,\alpha_2,\alpha_6 \in \{-1,1\}} p_1 + \min_{\alpha_4,\alpha_5,\alpha_7 \in \{-1,1\}} p_2
\end{align*}
where $p_1 = a_1 \alpha_1\alpha_2 + a_3\alpha_2\alpha_6 $ and $p_2 = a_2\alpha_4\alpha_5 + a_4\alpha_5\alpha_7$
The similar result holds when $\alpha_3 = -1$
\end{example}
